Mini-batch Serialization: CNN Training with Inter-layer Data Reuse

Training convolutional neural networks (CNNs) requires intense computations and high memory bandwidth. We find that bandwidth today is over-provisioned because most memory accesses in CNN training can be eliminated by rearranging computation to better utilize on-chip buffers and avoid traffic resulting from large per-layer memory footprints. We introduce the MBS CNN training approach that significantly reduces memory traffic by partially serializing mini-batch processing across groups of layers. This optimizes reuse within on-chip buffers and balances both intra-layer and inter-layer reuse. We also introduce the WaveCore CNN training accelerator that effectively trains CNNs in the MBS approach with high functional-unit utilization. Combined, WaveCore and MBS reduce DRAM traffic by 75%, improve performance by 53%, and save 26% system energy for modern deep CNN training compared to conventional training mechanisms and accelerators.

==> Makefile <==
all:  main.tex bib/*.bib
	pdflatex main
	bibtex main
	pdflatex main
	pdflatex -synctex=-1 main
	#sed -i -e 's/build_tex/tex/g' -e 's/\/cygdrive\/c/C:/g' main.synctex
	#gs -sOutputFile=main_bw.pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -dNOPAUSE -dBATCH main.pdf
clean: 
	rm -rf *.aux *.bbl *.blg *.log *.out *.synctex main.pdf main_bw.pdf main.dvi


==> tex/background.tex <==
\section{background}
\label{sec:background}

\subsection{CNN Architecture}
\label{sub_sec:cnn_arch}
% CNN architecture: CNN components
CNNs consist of various types of layers (\fig{fig:cnn}):
convolution layers extract feature maps (or activation) from input images, pooling layers reduce feature dimension, and fully-connected (FC) layers generate prediction score for each class.
A convolution layer typically includes feature normalization and activation.
Feature normalization maintains stable feature distribution across layers and samples~\cite{ioffe2015batch}, and activation represented as ReLU~\cite{nair2010rectified} adds non-linearity to the learning function.

% CNN architecture: Tensor dimension
Each layer accepts input features and produces output features. As shown in \fig{fig:cnn}, each set of input and output features have four dimensions: the size of sample mini-batch \((N)\) which is 1 in the figure, the number of channels \((C)\), and the height \((H)\) and width \((W)\) of each feature. 
We use \(i\) and \(o\) to denote input and output, respectively.

%%%% DRAM System and Bank Organization                                                    
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.48\textwidth]{fig/cnn.pdf}
    \caption{Layer operators and the feature structure of a CNN architecture with mini-batch size 1}
    \label{fig:cnn}
  \vspace*{-3mm}
\end{figure}

% CNN architecture: Layer resource requirement
Convolution and FC layer computation consists primarily of matrix multiplication and accumulation, with overall computation dominated by the convlution layers.
As illustrated in \fig{fig:cnn}, a convolution layer convolves its input features by small filter matrices (each \(R \!\times\! S\)) with a possible non-unit stride. 
Filters hold learning parameters called weights and there are \(C_i \times C_o\) filter matrices that map the input and output channels.
After each convolution, the results are accumulated to a single output data point. 
The number of multiplies in one convolution layer is shown in \eq{eq:conv_comp}. 
We assume \(W_i=H_i\) and \(Pad\) indicates zero padding size around a input feature boundary.
\begin{equation}
\small
\label{eq:conv_comp}
\frac{Multiplies}{CONV\ Layer} = N \times \Big(\! \frac{H_i+2Pad-R+1}{Filter\ Stride} \!\Big)^2 \!\!\times (R \!\times\! S) \!\times\! C_i \!\times\! C_o 
\end{equation}
As the same filter is reused for convolving input features and the same input feature is reused to compute different output features, a convolution layer typically involves large data reuse and its performance is bottlenecked by the compute throughput~\cite{chen2017eyeriss}.

% CNN architecture: Memory bound layers 
Other layers, including pooling, activation, and normalization have low arithmetic intensity as their major function is element-wise vector computations~\cite{krizhevsky2012imagenet,ioffe2015batch}.
Therefore, their performance is generally restricted by data access bandwidth.

% CNN architecture: multi-branch modules => (Sum, Join, Concat points) Introduce the structure and data reuse pattern
\textit{\textbf{Multi-branch Network Modules.}}
Recent CNNs typically consist of multi-branch modules that enable deeper, more accurate networks~\cite{szegedy2015going,szegedy2017inception,he2016deep}.
The residual (\fig{fig:multi-branch}.a) and Inception modules (\fig{fig:multi-branch}.b) are the most representative multi-branch modules and minor variations of these modules is commonly used in many modern CNNs~\cite{hu2017squeeze,zagoruyko2016wide}.
A residual module has two branches whose outputs are accumulated when they merge while an inception module has numerous branches whose outputs are concatenated at a common node.
As the input at the branch divergence is used by all branches and the outputs at the join can be referred by other branches for reduction, the multi-branch modules exhibit data locality between branches.

% CNN architecture: Size of activation and weights at different stage of network
\textit{\textbf{Per-layer Memory Footprint.}}
Each layer's memory footprint is determined by the size of inter-layer stationary data (input and output features) and the size of its weights.
Generally, early layers in a CNN have larger feature maps due to the high resolution but a small number of channels (and hence weights).
On the other hand, later layers, after many pooling stages, have smaller feature maps but with more channels.
As pooling reduces both the height and width of a feature map, the overall size of inter-layer stationary data is large for the early layers.
On the other hand, the size of weights is larger for later layers as their size is proportional to the number of both input and output channels \((C_i \times C_o \times R \times S)\).

\subsection{CNN Training}
\label{sub_sec:cnn_train}
% Mini-Batch training
\textit{\textbf{Mini-batch SGD.}}
In CNN training, a network first takes in a mini-batch of input samples and attempts to predict the correct outputs using its current weights.
Then, it compares its outputs to the ground truth and computes their average loss \(J\) (or prediction error) for the entire mini-batch. 
After that, the stochastic gradient descent (SGD) algorithm is typically applied to calculate the gradient of the loss w.r.t. the weights, minimizing the loss at each layer.
Finally, the original weights are updated adding their gradient multiplied by a learning rate along with a specific optimization algorithm~\cite{ruder2016overview}.

Commonly used mini-batch sizes range 32--512 samples (distributed to processors). Using a large mini-batch has two main advantages. First, a large mini-batch reduces the variance in parameter values between training steps and reduce the model parameter update frequency per epoch, saving training iterations and thus time and energy~\cite{li2014efficient,goyal2017accurate}.
Second, a larger mini-batch provides more data parallelism thus increases compute unit utilization and helps in distributed computing environment~\cite{das2016distributed}.

%%%% Multi-branch modules
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.47\textwidth]{fig/multi-branch.pdf}
    \caption{Network structure of multi-branch modules (Residual module and Inception module v4.b)}
    \label{fig:multi-branch}
  \vspace*{-3mm}
\end{figure}

%%%% Data reuse in training
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.44\textwidth]{fig/train.pdf}
    %\caption{Dataflow between layers in forward and backward propagations. The inter-layer stationary data are red and blue colored}
    \caption{Dataflow in forward- and back-propagations. Red arrows show the inter-layer reusable data}
    \label{fig:train}
  \vspace*{-3mm}
\end{figure}

% Forward and backward propagation
\sk{
The CNN training process consists of forward and backward network propagations as shown in \fig{fig:train} ($\phi$ indicates activation function).
First, the forward phase propagates the input data through layers to extract activations.
The extracted activation \((z)\) and the input to normalization layers \((x)\) are check-pointed to the off-chip memory as they get reused in the backpropagation to compute gradients at each layer.
Then, the backward phase propagates the gradient of the loss \((\frac{\partial J}{\partial edge_l})\) through layers and compute the gradients of weights at each convolution layer \((\frac{\partial J}{\partial w_{l}} )\).
%Here, \(d\) and \(W\) indicate activation and weights respectively. 
%These backward gradient equations are formulated as \eq{eq:backprop} for convolution layers (\(A'\) indicates activation function derivative).
%As illustrated in \fig{fig:train}, layer operators in the backward phase refer data between these two equations (colored data pairs) showing bigger data reuse opportunities than the forward phase.

The backpropagation involves bigger inter-layer reuse opportunity than the forward propagation.
Within each convolution layer, the upstream loss gradient is reused to compute both the weight gradient and the loss gradient of next layer.
To compute the gradient of activation, ReLU reuses the activation \((z)\) read in the previous convolution layer from memory.
Also, normalization layer reuses the check-pointed input data \(x\) and the upstream loss gradient multiple times to compute the gradient of parameters (scale and shift) and the loss gradient of the next layer~\cite{ioffe2015batch}.
%\begin{equation}
%\label{eq:backprop}
%\delta_{l-1} \!=\! (\delta_l \ast W_l^T)\circ A_l', \ \ \ \ \nabla W_l \!=\! A_{l-1} \ast \delta_l^T
%\end{equation}
}

\subsection{Feature Normalization}
\label{sub_sec:norm}
Feature normalization is critical to scaling deep network architectures and enabling faster convergence of the SGD algorithm~\cite{ioffe2015batch}. 
It maintains a constant feature distribution for the input to each convolution layer so avoids the parameter variance caused by random sample data distribution. 
Batch Normalization (BN) is the default technique for most modern deep CNNs and does this by normalizing data across mini-batch.
After normalization, BN scales and shifts the normalized data using per-channel learning parameters.
BN typically uses at least 32 or 64 samples (partial mini-batch assigned to a processor) for normalization.
The performance of BN is highly memory bound because each of the mean, variance, and normalization steps requires a read of the entire mini-batch.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.36\textwidth]{fig/norm.pdf}
    %\caption{Feature normalization structure of BN and GN (number of groups = 2)}
    \caption{Feature normalization structure of BN and GN}
    \label{fig:norm}
  \vspace*{-3mm}
\end{figure}

% Group Norm
As BN requires large mini-batch, it cannot be used when the size of mini-batch is small.
To cope with such problem, Group Normalization (GN) has been proposed~\cite{wu2018group}.
As shown in \fig{fig:norm}, GN divides channels \((C)\) into groups \((G)\) and normalizes data within \(C/G \!\times\! H \!\times\! W\) unlike to \(N \!\times\! H \!\times\! W\) of BN.
By normalizing data in the channel dimension, GN avoids the dependence to the size of mini-batch.
Their evaluation shows GN has similar prediction accuracy of BN regardless of the size of mini-batch.
Like BN, GN also does scale and shift the data after normalization using per-channel learning parameters.
The memory access and computation cost for GN is the same as BN given the same feature dimensions.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tex/locality_optimization.tex <==
\subsection{Locality Optimization}
\label{subsec:mbs_optimization}

\textit{\textbf{Sub-Batch Grouping Optimization.}}
\mattan{This procedure is not described well. I tried to describe what I thought could work, but I'm wrong. What you're doing is assuming max length is best and then merging back, but isn't it possible that some split mid-way is better? I left the text below half written until we figure this out.}
\mbs balances the reuse and locality of weights and features by choosing the sizes of sub-batches and layer group boundaries. Specifically, a new group is formed only if the weight reuse gained by increasing the sub-batch size reduces memory traffic compared to extending inter-layer reuse further, as captured by \eq{eq:sub_bath_group_fusion}. 
% Some sub-batch groups can be fused to save the activation reads from memory at sub-batch boundaries.
% However, this optimization has a trade-off as it reduces the sub-batch size of a group to match another's. 
% This results in increased weight re-fetches and reduced data parallelism for the group with reduced sub-batch size. 
% Thus, we fuse a sub-batch group only when the saved activation traffic is larger than the increased weight traffic.
% \eq{eq:sub_batch_group_fusion} enumerates the fusion condition.
\(D_{next}\), \(W_{next}\), \(L_{next}\) indicate the input feature data size, weight size, and maximum sub-batch length of the layer considered for starting a new group and  \(L_{curr}\) is the sub-batch length of the current group.
% \(ITERS\_DIFF\) calculates the difference in the number of sub-batch group iterations and \(L\) indicates the number of layers in a group.
Using this approach, the first, second, and third sub-batch groups in \fig{fig:mbs1} are combined to improve locality, vs. simply maximizing sub-batch size. 
\begin{equation}
\label{eq:sub_batch_group_fusion}
\small
\begin{split}
D_{next}(t) \!\times\! \frac{samples}{mini{\text -}batch} > \left(L_{next} - L_{prev}\right) \!\times\!\! \sum_{l\in L(t)} \!\!W_{l}
\end{split}
\end{equation}
\vspace*{-2mm}

\textit{\textbf{Inter-Iteration Weight Reuse.}}
\mattan{Can cut this section and save a lot of space. It's not all that important, is it?}
\mbs optimizes on-chip buffer utilization by keeping as many weights as possible in the buffer between sub-batch iterations. In early layers, this can result in substantial memory traffic reductions because many iterations are needed per group because of the large feautre sizes. \fig{fig:mbs2} shows how the global buffer of each block of ResNet50 is used for inter-layer data (features), various temporary data transferred from off-chip memory (block buffer), and weights that are reused across sub-batches. Similarly, the unused space or space indicated for weights is used in backward propagation to store weight gradients, which would otherwise be written to memory for later accumulation across an entire minibatch. 
% after sub-batch grouping optimization. After allocating the global buffer space to the inter-layer data and the blocking buffer for intra-layer weight reuse, a large space still remains unused.
% Given that layers in the early sub-batch group have a small number of weights, we can store their all their weights in the global buffer and reuse them across iterations.
% If the weights exceed the buffer capacity, a subset of the weights is stored, which still improves locality. 
%
% In backward propagation, \mbs involves an additional penalty: accumulating the weight gradients causes additional reads and writes. 
% Since weight gradient reduction causes more memory accesses than reading the weights, we use any remaining global buffer space for storing the partial weight gradients in backward phase.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.48\textwidth]{graph/mbs2.pdf}
    \vspace*{-7mm}
    \caption{Global buffer utilization in each block of ResNet50. Thick boxes indicate the sub-batch groups}
    \label{fig:mbs2}
  \vspace*{-4mm}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:



==> tex/motivation.tex <==
\section{motivation}
\label{sec:motivation}
%%%%% Importance of inter-layer stationary scheduling

%%%% DRAM System and Bank Organization                                                    
\begin{figure}[h]
\vspace*{-2mm}
    \centering
    \includegraphics[width=0.47\textwidth]{graph/footprint.pdf}
    \caption{The size of inter-layer stationary data and weights of each layer in ResNet50}
    \label{fig:footprint}
  \vspace*{-3mm}
\end{figure}

% Opportunity for data reuse in training and the problem by the large batch size
\fig{fig:footprint} shows the size of the inter-layer data and weights of every layer in ResNet50~\cite{he2016deep} in forward propagation phase.
Given per-processor partial mini-batch size 32 and word size 2B, the size of inter-layer data is much bigger than the weights. 
This infers the importance of capturing the locality between layers for training compared to the inference where the size of weights could be bigger than the reusable data between layers. 
However, due to their large footprint size, only 22\% of inter-layer data is reusable even with 20MB on-chip storage. 
This problem is further exacerbated if larger per processor mini-batch sizes are used as the inter-layer data footprint will increase as well. 
Therefore, it is critical to reduce the inter-layer data footprint of network layers to the on-chip buffer size. 
At the same time, this must be done without affecting the CNN functional correctness or reducing the hardware resource utilization.

